Iterative Document Representation Learning Towards Summarization with Polishing

In this paper, we introduce Iterative Text Summarization (ITS), an iteration-based model for supervised extractive text summarization, inspired by the observation that it is often necessary for a human to read an article multiple times in order to fully understand and summarize its contents. Current summarization approaches read through a document only once to generate a document representation, resulting in a sub-optimal representation. To address this issue we introduce a model which iteratively polishes the document representation on many passes through the document. As part of our model, we also introduce a selective reading mechanism that decides more accurately the extent to which each sentence in the model should be updated. Experimental results on the CNN/DailyMail and DUC2002 datasets demonstrate that our model significantly outperforms state-of-the-art extractive systems when evaluated by machines and by humans.

==> analysis.tex <==
\section{Results}



\begin{table}[t!]
	\begin{center}
		\begin{tabular}{l|ccc}
			\hline DailyMail &  Rouge-1 &  Rouge-2 &  Rouge-L\\ 
			\hline
			Lead-3 & 21.9 & 7.2 & 11.6 \\
			LReg(500) & 18.5 & 6.9 & 10.2 \\
			Cheng \emph{et.al}'16  & 22.7 & 8.5 & 12.5 \\
			SummaRuNNer & 26.2 & 10.8 & 14.4 \\
			\bf Our Method & \bf 27.4 & \bf 11.9 & \bf 16.2 \\
			\hline
		\end{tabular}
	\end{center}
	\caption{\label{tab:compare-baseline} Comparison with other baselines on Daily Mail test dataset using Rouge recall score with respect to the abstractive ground truth at 75 bytes. Scores are statistically significant using 95\% confidence interval as estimated by Rouge script.}
\end{table}

\begin{table}[t!]
	\begin{center}
		\begin{tabular}{l|ccc}
			\hline DailyMail &  Rouge-1 &  Rouge-2 &  Rouge-L\\ 
			\hline
			Lead-3 & 40.5 & 14.9 & 32.6 \\
			Cheng \emph{et.al}'16  &  42.2 &  17.3 &  \bf 34.8 \\
			SummaRuNNer & 42 & 16.9 & 34.1 \\
			\bf Our Method & \bf 42.3 & \bf 17.4 & 34.1 \\
			\hline
		\end{tabular}
	\end{center}
	\caption{\label{tab:b275} Comparison with other baselines on Daily Mail test dataset using Rouge recall score with respect to the abstractive ground truth at 275 bytes. Scores are statistically significant using 95\% confidence interval as estimated by Rouge script.}
\end{table}

Table \ref{tab:compare-baseline}  and table \ref{tab:b275} shows the performance comparison of our model with other baselines including \cite{Cheng2016Neural} and \cite{Nallapati2016SummaRuNNer} on the DailyMail corpus with respect to Rouge score at 75 bytes and 275 bytes of summary length. 
Our model performs consistently and significantly better than other models on 75 bytes.
while on 275 bytes, the improvement margin is smaller.
One possible interpretation is that our model has high precision on top rank outputs, but the confidence is lower for sentences. 
What's more, in \cite{Cheng2016Neural}, they used additional supervised training to create sentence-level extractive labels to train their model.

In Table \ref{tab:compare-duc}, we present the performance of model using the same metric on an out of domain corpus, DUC dataset. 
Our model outperforms other baselines in Rouge-2 and Rouge-L metric but underperforms state of the art model in \cite{Wan2010Towards} which are graph-based.
One possible reason for our model not consistently performing so well is that, our model is a supervised deep neural based model which can perform well on corpus it is trained on, but has adaptation problems when tested on a different domain corpus.

\begin{table}[t!]
	\begin{center}
		\begin{tabular}{l|ccc}
			\hline \bf DUC & \bf Rouge-1 & \bf Rouge-2 & \bf Rouge-L\\ 
			\hline
			Lead-3 & 43.6 & 21.0 & 40.6 \\
			LReg & 43.8 & 20.7 & 40.3 \\
			ILP & 45.4 & 21.3 & 42.8 \\
			Cheng \emph{et.al}'16  & 47.4 & 23.0 & \bf 43.5 \\
			SummaRuNNer  & 46.6 & 23.1 & 43.0 \\
			\bf Our Method & 47.1 & \bf 23.5 & \bf 43.5 \\
			\hline
		\end{tabular}
	\end{center}
	\caption{\label{tab:compare-duc} Comparison results on DUC test dataset using Rouge F-score with respect to the abstractive ground truth at 75 bytes. Scores are statistically significant using 95\% confidence interval as estimated by Rouge script.}
\end{table}


\subsection{Qualitative Analysis}

In this section, we first give a comparison example of gold summary and summary selected by our model. 

\begin{table}[t!]
	\begin{center}
		\begin{tabular}{|p{0.9\columnwidth}|}
			\hline
			\textbf{Gold Summary}: \\
			{\small @entity1 @entity0 was member of armed gang that targeted businesses
				
				criminals carried out 29 robberies and burglaries in @entity7
				
				@entity0 posted pictures of stolen cash and drugs on @entity5 profile} \\
			
			\hline
			\textbf{Our Method}: \\
			{\small jailed : @entity1 @entity0 posted pictures of stolen money and drugs on @entity5 after targeting businesses across @entity7 a 24-year-old man who carried out a series of raids on petrol stations and convenience stores has been jailed after boasting about his crimes on @entity5
				
				@entity1 @entity0 posted pictures of stolen money and drugs on the social networking site after targeting businesses across @entity7
				
				above, a @entity5 photograph that appears to show a stash of the drug prosecutor @entity76 told the court that on one occasion, the men stole nearly \pounds4,000 worth of cigarettes and \pounds1,000 in cash from a @entity83 garage in @entity84} \\
			\hline
		\end{tabular}
	\end{center}
	\caption{\label{tab:case} Example summary from a document of Daily Mail corpus.}
\end{table}

From the golden summary, we can have a overall concept that the article is about a business crime and stolen things have been posted. 
In the summary produced by our method, we can still sum up above information but get to know redundancies such as how young is the stealer, what things has he stolen. 
This weakness is due to the fact that out model can only extract original sentences, which unavoidably, might have unnecessary information.


\begin{figure} \centering
	\subfigure[{}] { \label{fig:logits1}     
		\includegraphics[width=\columnwidth]{img/logits1.pdf}
	}       
	\subfigure[{}] { \label{fig:logits2}
		\includegraphics[width=\columnwidth]{img/logits2.pdf}
	}  
	\caption{\label{fig:logits} The predicted score for each sentence calculated by the output of each iteration} 
\end{figure}

Next, to fully investigate the selecting probability distribution of each iteration, we pick two cases to show how the iterative method influences selecting sentence in Fig.\ref{fig:logits}. 
It presents the predicted score for each sentence calculated by the output of each iteration.
%The darker the color is, the more likely the sentence is selected. 
In Fig.\ref{fig:logits}(a), it can be seen that when the iteration just begins, most sentences have similar scores.
But when the iteration keeps processing, scores of some sentences begin to falling, and others are approaching the maximum value, which means that the model already has preferred sentence to be selected. 
Another interesting feature can be found in Fig.\ref{fig:logits}(b), we notice that there is a transitivity between passes. 
To be specific, the sentences which are not preferred by pass3 remain low scores in the next two passes, while sentences with relative high scores are still preferred by pass4 and pass5.
